On streaming approximation algorithms for constraint satisfaction problems

In this thesis, we explore streaming algorithms for approximating constraint satisfaction problems (CSPs). The setup is roughly the following: A computer has limited memory space, sees a long "stream" of local constraints on a set of variables, and tries to estimate how many of the constraints may be simultaneously satisfied. The past ten years have seen a number of works in this area, and this thesis includes both expository material and novel contributions. Throughout, we emphasize connections to the broader theories of CSPs, approximability, and streaming models, and highlight interesting open problems. The first part of our thesis is expository: We present aspects of previous works that completely characterize the approximability of specific CSPs like Max-Cut and Max-Dicut with $\sqrt{n}$-space streaming algorithm (on $n$-variable instances), while characterizing the approximability of all CSPs in $\sqrt n$ space in the special case of "composable" (i.e., sketching) algorithms, and of a particular subclass of CSPs with linear-space streaming algorithms. In the second part of the thesis, we present two of our own joint works. We begin with a work with Madhu Sudan and Santhoshini Velusamy in which we prove linear-space streaming approximation-resistance for all ordering CSPs (OCSPs), which are "CSP-like" problems maximizing over sets of permutations. Next, we present joint work with Joanna Boyland, Michael Hwang, Tarun Prasad, and Santhoshini Velusamy in which we investigate the $\sqrt n$-space streaming approximability of symmetric Boolean CSPs with negations. We give explicit $\sqrt n$-space sketching approximability ratios for several families of CSPs, including Max-$k$AND; develop simpler optimal sketching approximation algorithms for threshold predicates; and show that previous lower bounds fail to characterize the $\sqrt n$-space streaming approximability of Max-$3$AND.

==> endmatter/colophon.tex <==

\newpage

% If you do want an image in the colophon:
\begin{figure}
  \vspace{20pt}
  \centering
  \hspace*{-32pt}
  \includegraphics[width=0.42\textwidth]{endmatter/colophon.png}
\end{figure}

% If you don't want an image in the colophon:
% \vspace*{200pt}

\begin{center}
\parbox{200pt}{\lettrine[lines=3,slope=-2pt,nindent=-4pt]{\textcolor{SchoolColor}{T}}{his thesis was typeset} using \LaTeX, originally developed by Leslie Lamport and based on Donald Knuth's \TeX. The above illustration, \textit{Science Experiment 02}, was created by Ben Schlitter and released under \href{http://creativecommons.org/licenses/by-nc-nd/3.0/}{\textsc{cc by-nc-nd 3.0}}. A template that can be used to format a PhD dissertation with this look \textit{\&} feel has been released under the permissive \textsc{agpl} license, and can be found online at \href{https://github.com/suchow/Dissertate}{github.com/suchow/Dissertate} or from its lead author, Jordan Suchow, at \href{mailto:suchow@post.harvard.edu}{suchow@post.harvard.edu}.}
\end{center}


==> endmatter/notation.tex <==

% the abstract

\addcontentsline{not}{chapter}{Glossary}
\chapter*{Glossary}

\section*{Notations}

\begin{tabularx}{\textwidth}{@{}XX@{}}
  $k$ & arity of CSP/hypergraph \\
  $i$ & variable index ($\in [n]$) \\
  $\ell$ & edge index ($\in [m]$) \\
  $m$ & number of constraints/hyperedges \\
  $n$ & number of variables/vertices \\
  $q$ & alphabet size ($\in [m]$) \\
  $T$ & number of players/subinstances \\
  $[k]$ & natural numbers $\{1,\ldots,q\}$ \\
  $\BZ_q$ & group of integers modulo $q$ \\
  $f$ & predicate ($\BZ_q^k\to\{0,1\}$) \\
  $\CF$ & family of predicates \\
  $\alpha$ & constraint/hyperedge density (w.r.t. $n$) \\
  $\vecb$ & CSP predicate label/negation pattern \\
  $\vece$ & vertex-indices for hyperedge ($\in [n]^k$) \\
  $\vecj$ & variable-indices for constraint ($\in [n]^k$) \\
  $\vecx$ & CSP assignment ($\in \BZ_q^n$) \\
  $\vecx|_\vecj$ & projection of $\vecx$ onto coordinates $\vecj$ ($\in \BZ_q^k$) \\
  $\Unif_S$ & uniform distribution \\
  $\Matchings_{k,\alpha}(n)$ & $\Unif$ on $k$-hypermatchings \\
  $\Graphs_{k,\alpha}(n)$ & $\Unif$ on $k$-hypergraphs \\
  $\Bern_p$ & Bernoulli-$p$ distribution ($=0$ w.p. $p$, 1 o.w.) \\
  $M$ & vertex-hyperedge adjacency matrix \\
  $M^\fold$ & folded version of $M$ \\
  $\hat{f}(\vecs)$ & Fourier coefficient of $f$ \\
  $\1_S$ & indicator function for $S$ \\
  $\supp$ & support of vector/function/distribution \\
  $\sym_k$ & set of permutations on $[k]$ \\
  
\end{tabularx}

\section*{Abbreviations}

\begin{tabularx}{\textwidth}{@{}XX@{}}
  CSP & constraint satisfaction problem \\
  C2S & communication-to-streaming (reduction) \\
  SDP & semidefinite programming \\
  UGC & unique games conjecture \\
\end{tabularx}

\section*{Communication games}
\begin{tabularx}{\textwidth}{@{}XX@{}}
  $\bpd$ & Boolean partition detection \\
  $\seqbpd$ & sequential $\bpd$ \\
  $\seqibpd$ & implicit $\seqbpd$ \\
  $\rmd$ & randomized mask detection \\
  $\seqrmd$ & sequential $\rmd$ \\
  $\seqirsd$ & sequential implicit randomized shift detection
\end{tabularx}

==> endmatter/personalize.tex <==



==> frontmatter/abstract.tex <==

% the abstract

% ``The thesis should contain an informative abstract separate from the body of the thesis. This abstract should clearly state what the contribution of the thesis is–which parts are expository, whether there are novel results, etc. ''

In this thesis, we explore \emph{streaming algorithms} for \emph{approximating} \emph{constraint satisfaction problems (CSPs)}. The setup is roughly the following: A computer has limited memory space, sees a long ``stream'' of local constraints on a set of variables, and tries to estimate how many of the constraints may be simultaneously satisfied. The past ten years have seen a number of works in this area, and this thesis includes both expository material and novel contributions. Throughout, we emphasize connections to the broader theories of CSPs, approximability, and streaming models, and highlight interesting open problems.

The first part of our thesis is expository: We present aspects of previous works that completely characterize the approximability of specific CSPs like $\mcut$ and $\mdcut$ with $\sqrt{n}$-space streaming algorithm (on $n$-variable instances), while characterizing the approximability of all CSPs in $\sqrt n$ space in the special case of ``composable'' (i.e., \emph{sketching}) algorithms, and of a particular subclass of CSPs with \emph{linear-space} streaming algorithms.

In the second part of the thesis, we present two of our own joint works. We begin with a work with Madhu Sudan and Santhoshini Velusamy in which we prove linear-space streaming approximation-resistance for all \emph{ordering CSPs (OCSPs)}, which ``CSP-like'' problems maximizing over sets of permutations. Previous works considered the \emph{maximum acyclic subgraph} problem ($\mas$), the prototypical OCSP; even for $\mas$, we improve on both the inapproximability factor and the space bound.

Next, we present joint work with Joanna Boyland, Michael Hwang, Tarun Prasad, and Santhoshini Velusamy in which we investigate the $\sqrt n$-space streaming approximability of Boolean CSPs with negations. In particular, we give explicit $\sqrt n$-space sketching approximability ratios for several families of CSPs, including $\mkand$; develop simpler optimal sketching approximation algorithms for \emph{threshold} predicates; and show that previous streaming lower bounds are ``incomplete'' in that they fail to characterize the $\sqrt n$-space streaming approximability of $\mthreeand$.


==> frontmatter/authorlist.tex <==




==> frontmatter/dedication.tex <==

% dedication text

\textsc{To my parents and grandparents.}

\vspace{2in}

\epigraph{Program a map to display frequency of data exchange, every thousand megabytes a single pixel on a very large screen. Manhattan and Atlanta burn solid white. Then they start to pulse, the rate of traffic threatening to overload your simulation. Your map is about to go nova. Cool it down. Up your scale. Each pixel a million megabytes. At a hundred million megabytes per second, you begin to make out certain blocks in midtown Manhattan, outlines of hundred-year-old industrial parks ringing the old core of Atlanta$\ldots$}{William Gibson, \emph{Neuromancer}}

\epigraph{También se descifró el contenido: nociones de análisis combinatorico, ilustradas por ejemplos de variaciones con repetición ilimitada... Observó que todos los libros, por diversos que sean, constan de elementos iguales: el espacio, el punto, la coma, las veintidós letras del alfabeto.}{Jorge Luis Borges, ``La biblioteca de Babel''}

==> frontmatter/epigraphs.tex <==
\epigraph{Program a map to display frequency of data exchange, every thousand megabytes a single pixel on a very large screen. Manhattan and Atlanta burn solid white. Then they start to pulse, the rate of traffic threatening to overload your simulation. Your map is about to go nova. Cool it down. Up your scale. Each pixel a million megabytes. At a hundred million megabytes per second, you begin to make out certain blocks in midtown Manhattan, outlines of hundred-year-old industrial parks ringing the old core of Atlanta$\ldots$}{William Gibson, \emph{Neuromancer}}

\epigraph{\emph{También se descifró el contenido: nociones de análisis combinatorico, ilustrados por ejemplos de variaciones con repetición ilimitada... Observó que todos los libros, por diversos que sean, constan de elementos iguales: el espacio, el punto, la coma, las veintidós letras del alfabeta.}}{Jorge Luis Borges, \emph{Ficciones}}

==> frontmatter/thanks.tex <==

% the acknowledgments section

I am deeply grateful to Madhu Sudan for being a wonderfully supportive research advisor and all-around mentor throughout my time at Harvard. I've fortunate to have had the opportunity to work with and learn from him, and I'm still amazed at his patience and generosity in responding to my seemingly never-ending Slack messages, and providing a similarly never-ending stream of advice, feedback, and insights.

Santhoshini Velusamy has been a fantastic collaborator on both joint works presented in this thesis \cite{SSV21,BHP+22}. Her suggestion to work on streaming algorithms for the $\mas$ problem, an interesting question left open from her own undergraduate research internship (cf. \cite{GVV17}), kicked off my work on streaming CSPs which, almost two years later, has blossomed into this thesis. (\cref{chap:ocsps} presents joint work with Madhu \cite{SSV21} which includes a resolution of her original question.) Thanks also to my other coauthors on our joint work \cite{BHP+22} (\cref{chap:sym-bool}): Joanna Boyland, Tarun Prasad, and Michael Hwang; to Sumegha Garg, Chi-Ning Chou, Sasha Golovnev, Ameya Velingker, and Raghuvansh Saxena for helpful insights and discussions; and to the Harvard College Research Program for supporting my work on \cite{BHP+22} in Fall 2021.

Thank you to Salil Vadhan for being my second thesis reader; to Boaz Barak for his years of advice and encouragement, beginning with a welcoming and friendly series of emails about CS at Harvard which, as much as anything, convinced me to attend; and to Eric Allender for being a wonderful mentor during the DIMACS REU program at Rutgers over Summer 2021. Additionally, I am grateful for the deeply influential experience of serving as an undergraduate Teaching Fellow (TF) in courses taught by Madhu and Boaz as well as Adam Hesterberg, James Mickens, and Michael Mitzenmacher.

Finally, I would like to thank my parents Mindy Weinstein and Joel Singer, my brother Ethan, the rest of my family, and many friends including Braxton Marion, Clara Li, James Roney, Joshua Doolan, Jyotsna Rao, Nari Johnson, Shuvom Sadhuka, and Sahana Srinivasan for providing immeasurable support on my journey throughout college towards research and graduate school.
